Heart Artifact Removal in Electrohysterography Measurements Using Algebraic Differentiators

Electrohysterography (EHG) enables non-invasive monitoring of uterine contractions but can be contaminated by electrocardiogram (ECG) artifacts. This work presents an ECG removal method using algebraic differentiators, a control-theoretic tool for model-free derivative estimation, that preserves signal shape outside the detected cardiac pulse locations. The differentiator parameters are designed to simultaneously suppress slow physiological artifacts and powerline interference. Cross-channel clustering distinguishes cardiac pulses from localized artifacts, enabling accurate pulse subtraction without auxiliary ECG references. Implemented as a causal FIR filter, the method is validated as a proof of concept on multichannel EHG recordings from one female and one male healthy volunteer and compared to the template subtraction method.

==> robustExternalize/robExt-61FE73C5A0756E29C9E9A30AAEB152FE-out.tex <==
\def\robExtWidth{225.38364pt}\def\robExtHeight{156.93428pt}\def\robExtDepth{0.0pt}


==> robustExternalize/robExt-94376F8F1A0B10A6985C2BF3DF7AC3D3-out.tex <==
\def\robExtWidth{219.20958pt}\def\robExtHeight{156.93599pt}\def\robExtDepth{0.0pt}


==> robustExternalize/robExt-B42DAE292581D3B6EE0795C08383ACA6-out.tex <==
\def\robExtWidth{226.96388pt}\def\robExtHeight{156.9315pt}\def\robExtDepth{0.0pt}


==> robustExternalize/robExt-C809B31588AF392E928890FB2713D41F-out.tex <==
\def\robExtWidth{192.83994pt}\def\robExtHeight{101.60104pt}\def\robExtDepth{0.0pt}

